An Assessment of the Usability of Machine Learning Based Tools for the Security Operations Center

Gartner, a large research and advisory company, anticipates that by 2024 80% of security operation centers (SOCs) will use machine learning (ML) based solutions to enhance their operations. In light of such widespread adoption, it is vital for the research community to identify and address usability concerns. This work presents the results of the first in situ usability assessment of ML-based tools. With the support of the US Navy, we leveraged the national cyber range, a large, air-gapped cyber testbed equipped with state-of-the-art network and user emulation capabilities, to study six US Naval SOC analysts' usage of two tools. Our analysis identified several serious usability issues, including multiple violations of established usability heuristics form user interface design. We also discovered that analysts lacked a clear mental model of how these tools generate scores, resulting in mistrust and/or misuse of the tools themselves. Surprisingly, we found no correlation between analysts' level of education or years of experience and their performance with either tool, suggesting that other factors such as prior background knowledge or personality play a significant role in ML-based tool usage. Our findings demonstrate that ML-based security tool vendors must put a renewed focus on working with analysts, both experienced and inexperienced, to ensure that their systems are usable and useful in real-world security operations settings.

==> 90-conclusion.tex <==
\section{Future Work}
% more tools - more goodness - etc.
We plan to continue this work in several ways. 
First, we want to 










==> 97-acks.tex <==

\section*{Acknowledgments}
The authors thank all security analysts that agreed to
participate in this study and the team at the National Cyber Range, without whom this study would not have been possible. [Rest of acknowledgements
redacted for double-blind review.]

